Efficient Pruning for Machine Learning Under Homomorphic Encryption

Privacy-preserving machine learning (PPML) solutions are gaining widespread popularity. Among these, many rely on homomorphic encryption (HE) that offers confidentiality of the model and the data, but at the cost of large latency and memory requirements. Pruning neural network (NN) parameters improves latency and memory in plaintext ML but has little impact if directly applied to HE-based PPML. We introduce a framework called HE-PEx that comprises new pruning methods, on top of a packing technique called tile tensors, for reducing the latency and memory of PPML inference. HE-PEx uses permutations to prune additional ciphertexts, and expansion to recover inference loss. We demonstrate the effectiveness of our methods for pruning fully-connected and convolutional layers in NNs on PPML tasks, namely, image compression, denoising, and classification, with autoencoders, multilayer perceptrons (MLPs) and convolutional neural networks (CNNs). We implement and deploy our networks atop a framework called HElayers, which shows a 10-35% improvement in inference speed and a 17-35% decrease in memory requirement over the unpruned network, corresponding to 33-65% fewer ciphertexts, within a 2.5% degradation in inference accuracy over the unpruned network. Compared to the state-of-the-art pruning technique for PPML, our techniques generate networks with 70% fewer ciphertexts, on average, for the same degradation limit.

==> 07_discussion.tex <==
\section{Discussion}\label{sec:discussion}

\mysec{Supporting non-FC Layers} 
This work demonstrated \FRAME for networks with \gls{FC} and activation layers to showcase a focused set of experiments and analyses.
However, this does not imply that our methods are not applicable to other layers, such as convolutional layers.
Particularly, we did not evaluate \FRAME with convolutional layers because the fact that convolution filters are generally small, it becomes less interesting to do pruning, permutation and expansion on them.
However, HElayers \cite{helayers} uses a different convolutional packing method than GAZELLE \cite{GAZELLE2018}. 
It would be interesting to compare the effect of pruning \glspl{CNN} using our proposed approaches and comparing with other work such as Hunter~\cite{hunter}. 
We leave this effort for a future work.

\mysec{Tackling the Drawbacks of Non-Interactive Solutions}
A common claim in favor of client-aided solutions over non-client-aided ones is that they do not require training a new network, \ie the data model can use an off-the-shelf network, even if it includes non-linear operations that can be executed securely by the client. 
Clearly, this claim no longer holds when considering client-aided solutions such as Hunter~\cite{hunter}, as the model owner needs to prune and retrain the network. 
In that sense, the cost of also considering \gls{HE}-friendly layers, \ie only linear operations, becomes negligible, which gets the community one step ahead toward having usable non-interactive \gls{HE}-based solutions. 


==> fig_ourmethods_small.tex <==
 \begin{figure}[t!]
    \scriptsize
    \begin{minipage}[t]{0.48\linewidth}
    \begin{align*}
        & \meth{P2}: \hspace{-10pt} & \operatorname{Train} & \rightarrow \operatorname{\underline{P}rune} \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack} \\[0pt]
        & \meth{P2T}: \hspace{-10pt} & \operatorname{Train} & \rightarrow \operatorname{\underline{\bf P}rune\textsuperscript{\underline{\bf t}ile}} \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack} \\[0pt]
        & \meth{P3}: \hspace{-10pt} &  \operatorname{Train} & \rightarrow \operatorname{\underline{\bf P}rune} \rightarrow \operatorname{\underline{\bf P}ermute} \rightarrow & \\[0pt]
        & & & \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack}\\[0pt]
        & \meth{P3E}: \hspace{-10pt} & \operatorname{Train} & \rightarrow \operatorname{\underline{\bf P}rune} \rightarrow \operatorname{\underline{\bf P}ermute} \rightarrow & \\[0pt]
        & & & \rightarrow \operatorname{\underline{\bf E}xpand} \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack} \\[0pt]
        & \meth{P4}: \hspace{-10pt} &  \operatorname{Train} & \rightarrow \operatorname{\underline{\bf P}rune} \rightarrow \operatorname{\underline{\bf P}ermute} \rightarrow \\[0pt]
        & & & \rightarrow \operatorname{\underline{\bf P}rune\textsuperscript{pack}}\hspace{-5pt} \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack} \\[0pt]
        & \meth{P4E}: \hspace{-10pt} & \operatorname{Train} & \rightarrow \operatorname{\underline{\bf P}rune} \rightarrow \operatorname{\underline{\bf P}ermute} \rightarrow  \operatorname{\underline{\bf P}rune\textsuperscript{pack}}  \rightarrow \\[0pt] 
        & & & \rightarrow \operatorname{\underline{\bf E}xpand} \rightarrow \operatorname{Retrain} \rightarrow \operatorname{\underline{\bf P}ack} \\[0pt]
    \end{align*}
    \caption{Overview of our prune, permute, expand, and pack methods.} % \hl{evaluated} as part of \FRAME.}
    \label{fig:ourmethods}
    \end{minipage}
\end{figure}
